Self-similar shock wave solutions of the non-linear Maxwell equations

In our study we consider nonlinear, power-law field-dependent electrical permitivity and magnetic permeability and investigate the time-dependent Maxwell equations with the self-similar Ansatz. This is a first-order hyperbolic PDE system which can conserve non-continuous initial conditions describing electromagnetic shock-waves. Besides shock-waves other interesting solutions (e.g. with localized compact support) can be found with delicate physical properties. Such phenomena may happen in complex materials induced by the planned powerful Extreme Light Infrastructure(ELI) laser pulses.

==> referee_riport_answer <==
Dear Madam/Sir,

First of all, we would like to thank the referee for his/her positive 
decision and for the constructive remarks. We corrected the manuscript 
according to his/her recommendations with our best knowledge. 

We answer now the questioned points:  

1. Author claims that his self-similar solutions are shock wave
solutions, in some cases , but not given the corresponding shock
boundary conditions which are satisfied by these solutions.
--After the defintion of the general form of the self-similar solutions, 
(9) we give an in depth analysis of these kind of solutions.  
The point is that this kind of solution cannot really incorporate a well-defined inital 
condition. In some cases the source type initial condition (Dirac delta) can be obtained 
but not everywhere.  


2. Author should check the sign of the second term on R.H.S. of the
first of equations (12). In my calculation, there should be plus in
place of minus. In this way, values of the various exponents should be
corrected. Also, the description of the solutions should be revised
accordingly.
--Yes, there was a missprint in the first equation (12). This was corrected. 
In the second next line the exponent is corrected as well. \beta = q+1.  
The whole calculation was checked and the final equation (14) was  
changed. The results become much more transparent.  
The essence of the paper however remained, there are two different physical regimes 
for different q exponents. There are continuous and shock-wave solutions of the problem. 
Figure 1a and 1b are changed to present the direction fields for the right results.   


3. There are two authors in the reference[3], but only one is quoted
in the Text. That should be corrected.
- Yes we wrote both names Zel'dovich and Raizer at the questioned point. 
We included some new references which we found in the last days. 

4. There are many misprints, and so the paper should be carefully
revised and corrected.
--We went throught the manuscript many times and corrected all the misprints we found.  
Some parts of the manuscript was reformulated as well.  





